Differentially Private Clustering: Tight Approximation Ratios

We study the task of differentially private clustering. For several basic clustering problems, including Euclidean DensestBall, 1-Cluster, k-means, and k-median, we give efficient differentially private algorithms that achieve essentially the same approximation ratios as those that can be obtained by any non-private algorithm, while incurring only small additive errors. This improves upon existing efficient algorithms that only achieve some large constant approximation factors. Our results also imply an improved algorithm for the Sample and Aggregate privacy framework. Furthermore, we show that one of the tools used in our 1-Cluster algorithm can be employed to get a faster quantum algorithm for ClosestPair in a moderate number of dimensions.

==> overview.tex <==
\section{Overview of Proofs}\label{subsec:overview_proofs}

\subsection{Stuff from Old Intro}

% \begin{theorem} \label{thm:main-apx-non-private-to-private-pure-intro}
% Suppose there is a polynomial-time (not necessarily private) $\rho$-approximation algorithm for $k$-medians (respectively, $k$-means) in Euclidean space. Then, for every $0 < \eps, \alpha < 1$, there is an $\eps$-DP algorithm that runs in time $k^{O_{\alpha}(1)} \poly(nd)$ and, with probability $0.99$, solves $k$-medians (respectively, $k$-means) with approximation ratio $\rho(1 + \alpha)$ and additive error $O_{\rho, \alpha}\left(\left(\frac{kd + k^{O_{\alpha}(1)}}{\eps}\right) \poly\log\left(\frac{n}{\eps}\right)\right)$.
% \end{theorem}

The next theorem guarantees an additive error smaller by a factor of $\sqrt{d}$ in the approximate DP case.
\begin{theorem} \label{thm:intro-apx-non-private-to-private-apx}
Suppose there is a polynomial-time (not necessarily private) $\rho$-approximation algorithm for $k$-medians (respectively, $k$-means) in Euclidean space. Then, for every $0 < \eps, \delta, \alpha < 1$, there is an $(\eps, \delta)$-DP algorithm that runs in time $k^{O_{\alpha}(1)} \poly(nd)$ and, with probability $0.99$, solves $k$-medians (respectively, $k$-means) with approximation ratio $\rho(1 + \alpha)$ and additive error $O_{\rho, \alpha}\left(\left(\frac{k\sqrt{d}}{\eps} \cdot \poly\log\left(\frac{k}{\delta}\right) \right) + \left(\frac{k^{O_{\alpha}(1)}}{\eps} \cdot \poly\log\left(\frac{n}{\eps}\right)\right)\right)$.
\end{theorem}


One approach for solving \textsf{DensestBall} is to run the Exponential Mechanism of McSherry and Talwar \cite{McSherryT07} on the $\alpha r$-covering of the unit ball, which would achieve an approximation ratio of $w = 1 + \alpha$ and incur an additive error of $t = \tilde{O}_{\eps}(d \log(1/r))$. The drawback of this approach is that it is inefficient: its running time is $O(\left(\frac{1}{\alpha r}\right)^d)$, which is super-polynomial.


We remark that, throughout this work, we will mainly state our guarantee for the case $\eps < 1$ for simplicity. All of our algorithms also work for $\eps \geq 1$, but the additive errors will change slightly. For example, additive errors in the above two theorems remain almost the same except that the $\eps$ term will disappear from the denominators in the $\poly\log$ terms.

\begin{theorem} \label{thm:fpt-cluster-pure-high-dim-intro}
For every $0 < \eps, \alpha < 1$, there is an $\eps$-DP algorithm that runs in time $2^{O_{\alpha}(k \log k)} \poly(nd)$ and, with probability $0.99$, solves $k$-means (respectively, $k$-medians) with approximation ratio $1 + \alpha$ and additive error $O_{\alpha}\left(\left(\frac{kd + k^2}{\eps}\right) \cdot \poly\log\left(\frac{n}{\eps}\right)\right)$.
\end{theorem}

Once again, we can further reduce the additive error if we settle for approximate DP.
\begin{theorem} \label{thm:fpt-cluster-apx-high-dim-intro}
For every $0 < \eps, \delta, \alpha < 1$, there is an $(\eps, \delta)$-DP algorithm that runs in time $2^{O_{\alpha}(k \log k)} \poly(nd)$ and, with probability $0.99$, solves $k$-means (respectively, $k$-medians) with approximation ratio $1 + \alpha$ and additive error $O_{\alpha}\left(\left(\frac{k\sqrt{d}}{\eps} \cdot \poly\log\left(\frac{k}{\delta}\right) \right) + \left(\frac{k^2}{\eps} \cdot \poly\log\left(\frac{n}{\eps}\right)\right)\right)$. 
\end{theorem}


=======

We next outline  the main ideas behind our results. While there are several technical details that we have to work out, a unifying theme that underlies our algorithms is that, by using dimensionality reduction and appropriate covers of the lower-dimensional space, we can devise efficient DP clustering algorithms which, up to small additive errors, achieve performance similar to their non-private counterparts.

\paragraph{Densest Ball} The crux of our algorithm for \textsf{DensestBall} is that, by using carefully selected tools, we can obtain an efficient implementation of the Exponential Mechanism. To explain our approach, we first recall the straightforward implementation of the Exponential Mechanism:
\begin{itemize}
    \item Consider any $\alpha r$-cover $C$ of the unit ball.
    \item For every $c \in C$, let $score[c]$ be the number of input points in $\cB(c, (1 + \alpha)r)$.
    \item Output a point $c^* \in C$ with probability $\frac{e^{(\eps/2) \cdot score[c^*]}}{\sum_{c \in C} e^{(\eps/2) \cdot score[c]}}$.
\end{itemize}
This algorithm is $\eps$-DP and gives a $1 + \alpha$ multiplicative approximation for the \textsf{DensestBall} problem. However, its drawback is that it runs in time $\poly(|C|)$, and $|C|$ has size at least $(\frac{1}{\alpha r})^d$ which is super-polynomial. 

First, observe that $d$ can be easily reduced to $O_\alpha(\log n)$ using generic dimensionality reduction techniques (e.g.,~\cite{JL}). Nonetheless, this is insufficient for our purposes as $\alpha r$ can be sub-constant. Indeed, in applications of \textsf{DensestBall} to $k$-means and $k$-medians clustering, $r$ will be as small as $O(1/n)$. Thus, mere dimensionality reduction would still lead to a super-polynomial running time. However, we note that if we consider an $\alpha r$-cover that is also an $\Omega(\alpha r)$-packing of the unit ball, then we can can bound the number of cover points $c \in C$ for which $score[c] > 0$ by $2^{O_\alpha(d)}$, which is polynomial whenever $d = O_\alpha(\log n)$ and $\alpha$ is an arbitrarily small positive constant. Intuitively, in order to obtain a polynomial time \textsf{DensestBall} algorithm, it suffices to prove that we can restrict the solution space in the Exponential Mechanism to these ``meaningful'' cover points. Doing so turned out to require overcoming the following two challenges:
\begin{itemize}
\item First, the Exponential Mechanism should still (by design) be able to sample every cover point in $C$, even the ``non-meaningful'' ones, with some positive probability. To this end, we show (in Section~\ref{sec:sparse-selection}) that such a procedure can be done efficiently, if either (i) we are allowed approximate DP (i.e., $\delta > 0$) or (ii) we can implement an efficient oracle for sampling cover points from $C$, and where each point has a non-trivial probability of being sampled.
\item Second, it is critical to the above approach that $C$ is both an $\alpha r$-cover and an $\Omega(\alpha r)$-packing. Straightforward choices of $C$, such as a maximal $(\alpha r / 2)$-packing, result in a construction time that is $\poly(|C|)$, which, as explained before, is insufficient for our purposes as it leads to a super-polynomial time algorithm for \textsf{DensestBall}. In fact, in the aforementioned case, it is not even clear how to represent $C$ compactly (in less than $|C|$ bits). Furthermore, given the input points $x_1, \dots, x_n$, it is unclear how to find ``meaningful'' cover points in $C$ without going through all the elements of $C$.
\end{itemize}
To solve these two issues, we resort to lattice-based packings, which exhibit two helpful properties for our purposes: cover points can be represented compactly in terms of the basis points, and the ``meaningful'' cover points can be efficiently found using powerful lattices algorithms (specifically, ones solving the so-called \emph{Closest Vector Problem}). The details are given in Section~\ref{sec:cover}.
% We note here that the cover that we use is well-known, and that our main contribution here is showing how to use it in the context of private clustering.
